Efficiently Checking Actual Causality with SAT Solving

Recent formal approaches towards causality have made the concept ready for incorporation into the technical world. However, causality reasoning is computationally hard; and no general algorithmic approach exists that efficiently infers the causes for effects. Thus, checking causality in the context of complex, multi-agent, and distributed socio-technical systems is a significant challenge. Therefore, we conceptualize an intelligent and novel algorithmic approach towards checking causality in acyclic causal models with binary variables, utilizing the optimization power in the solvers of the Boolean Satisfiability Problem (SAT). We present two SAT encodings, and an empirical evaluation of their efficiency and scalability. We show that causality is computed efficiently in less than 5 seconds for models that consist of more than 4000 variables.

==> sections/proof.tex <==

\begin{theorem}\label{theorem:F}
	Formula $F$ constructed within Algorithm.\ref{algorithm:fulfillsac2_sat} is satisfiable iff AC2 holds for a model $M$, context $\vec{u}$, an evaluation $\vec{V}=\vec{v}$ of endogenous variables, a tentative cause $\vec{X}=\vec{x}$, and a Boolean combination of primitive events $\varphi$. %This is denoted by SAT($F$) $\leftrightarrow$ AC2.
\end{theorem}

\begin{proof} The proof consists of two parts.
	\begin{proofpart}
		SAT($F$) $\implies$ AC2, AC2 holds if $F$ is satisfiable 
	\end{proofpart}
	We show this by contradiction. Assume that $F$ is satisfiable and AC2 does not hold. Based on $F$'s truth assignment, $\vec{v'}$, we cluster the variables  into 3 groups.

\vspace{-5mm}
\begin{align*}\label{eq:proof_f}
   \resizebox{1.0\hsize}{!}{%
	 $F := \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i) 	\wedge\bigwedge_{i=1\ldots\ell} f(X_i=\neg x_i)  \wedge\bigwedge_{i=1\ldots m, \not\exists j\bullet X_j=V_i} \left(V_i \leftrightarrow F_{V_i} \lor f(V_i=v_i)\right)$
	}
\end{align*}

	\noindent\textbf{1.} $\vec{X}$: each variable is fixed exactly to the negation of its original value, i.e.,  $\forall i X_i=\neg x_i \in \vec{V}=\vec{v'}$.	\textbf{2.} $\vec{W}^*$: variables in this group, if they exist, have equal truth  and original assignments, i.e., $\langle W^*_1,\ldots,W^*_s\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow W^*_i\not= W^*_j) \wedge (W^*_i=V_j\Leftrightarrow v_j'=v_j)$	\textbf{3.} $\vec{Z}$: variables in this group evaluate differently from their original evaluation, i.e., $ \langle Z_1,\ldots,Z_k\rangle$ s.t. $\forall i\forall j\bullet (i\not= j\Rightarrow Z_i\not= Z_j) \wedge (Z_i=V_j\Leftrightarrow v_j'\not= v_j) \wedge (\forall i\not\exists j\bullet Z_i=X_j$).  \\

\noindent Using $\vec{W^*},\vec{Z}$, we re-write $F$ as $F'$ which is  also satisfiable. 
\vspace{-2mm}
\begin{align*}
  \resizebox{1.0\hsize}{!}{%
$F' := \neg\varphi \wedge \bigwedge_{i=1\ldots n} f(U_i=u_i) 
\wedge\bigwedge_{i=1\ldots\ell} f(X_i=\neg x_i)
\wedge\bigwedge_{i=1\ldots s}  f(W^*_i=w^*_i)
\wedge\bigwedge_{i=1\ldots k} (Z_i \leftrightarrow F_{Z_i})$
}
\end{align*}
\vspace{-4mm}
%from here eith map to the causality model or go from the other side
%Since $M$ is acyclic, then there is a unique solution of the equations for a given context $\vec{u}$ \cite{halpern2016actual} that can be inferred from the formula.The truth assignment of the formula fixes values in $\vec{X}, \vec{W}, \vec{U}$ and leaves the other variables in $\vec{Z}$ to evaluate according to their equations, evaluating $\varphi$ to its negation.

\noindent Recall that $M$ is acyclic; therefore there is a unique solution to the equations. Let $\Psi$ be the equations in $M$ without the equations that define the variables $\vec{X}$. Let $\Psi_k$ be $\Psi$ without the equations of some variables in a set $\vec{W_k}$. Since AC2 does not hold, then $\forall k \bullet (\vec{W_k} \in  \mathcal{P}(V/X) \Rightarrow (\vec{X}=\vec{\neg x}\wedge\vec{W_k}=\vec{w_k} \wedge \Psi_k\wedge \neg\varphi)$ evaluates to \textit{false}, where $\mathcal{P}(V/\vec{X})$ is the power set of variables in $\mathcal{V}$ without variables in $\vec{X}$. In case $\vec{W_k} = \vec{W^*}$, the previous unsatisfiable formula is equivalent to the satisfiable $F'$, implying a contradiction.

\begin{proofpart}\label{lemma:f}
	 AC2 $\implies$ SAT($F$); $F$ is satisfiable if AC2 holds 
\end{proofpart}
	Assume that AC2 holds and $F$ is unsatisfiable. Then $\exists \vec{W},\vec{w},\vec{x}'\bullet  (M,\vec{u})\models(\vec{W}=\vec{w})
	\implies (M,\vec{u})\models\bigl[\vec{X}\leftarrow \vec{x}',\vec{W}\leftarrow\vec{w}\bigr]\neg\varphi$. According to \cite{halpern2015modification}, $(M, \vec{u}) \models [Y_1 \leftarrow y_1.. Y_k \leftarrow y_k]\varphi$ is equivalent to $(M_{Y_1 \leftarrow y_1..Y_k \leftarrow y_k}, \vec{u}) \models \varphi$, i.e., we replace specific equations in $M$ to obtain a new model $M' = M_{Y_1 \leftarrow y_1, ..., Y_k \leftarrow y_k}$. We replace the equations of the variables in $\vec{X},\vec{W}$ in $M$ to obtain a new model, $M'$, such that $(M',\vec{u})\models\neg\varphi$. The replaced equations are of the form $V_i=v_i$. $M'$ is acyclic and has a unique solution for $\vec{u}$. We construct a formula, $F'$ that is a conjunction of the variables in sets $X',W',$ and $U'$ in $M'$. Because of their equations, all these variables are represented as literals. Based on the nature of this formula, it will not contain two different literals for the same variable, and hence, it is satisfiable with exactly the same truth assignment as the unique solution of $M'$.   
	\vspace{-1mm}
\begin{small}
	\begin{align*}
	F' := \wedge \bigwedge_{i=1\ldots n} f(U_i'=u_i') 
	\wedge\bigwedge_{i=1\ldots s}  f(W_i'=w_i') 
	\wedge\bigwedge_{i=1\ldots\ell} f(X_i'= x_i')
	\end{align*}
\end{small}

	Now, we add the remaining variables, i.e., $\forall i \bullet V_i\notin(\vec{X}\cup\vec{W})$, as formulas using the $\leftrightarrow$ operator. The overall formula $F''$, is satisfiable because we have an assignment that makes each equivalence relation true.
 \begin{small}
	\begin{align*}
	F'' :=  F' \wedge \bigwedge_{i=1\ldots m, \not\exists j\bullet X_j=V_i, W_j=V_i}  (V_i \leftrightarrow F_{V_i})
	\end{align*}
\end{small}
	We have $(M',\vec{u})\models\neg\varphi$, which says that the model evaluates $\neg\varphi$ to true with its unique solution (same assignment of $F''$). We add another clause to $F''$ which evaluates to true and keeps the formula satisfiable. That is, $ F''' :=  F'' \wedge \neg\varphi$. Last, we only have to show the relation between ($F$ and  $F'''$). We can rewrite $F$ (shown at the beginning of the proof) such that we remove all disjuncts of the form $(V_i \leftrightarrow F_{V_i})$ for the variables in $\vec{W}$. Similarly, we remove  all disjuncts of the form $f(V_i=v_i)$ for all the variables that are not in $\vec{W}$. According to our assumption, $F$ is still unsatisfiable, since we removed disjunctions from the clauses. This contradicts the result we obtained from $F'''$ which is satisfiable for the same clauses. 
\end{proof}

